Zero-shot Depth Completion via Test-time Alignment with Affine-invariant Depth Prior

Depth completion, predicting dense depth maps from sparse depth measurements, is an ill-posed problem requiring prior knowledge. Recent methods adopt learning-based approaches to implicitly capture priors, but the priors primarily fit in-domain data and do not generalize well to out-of-domain scenarios. To address this, we propose a zero-shot depth completion method composed of an affine-invariant depth diffusion model and test-time alignment. We use pre-trained depth diffusion models as depth prior knowledge, which implicitly understand how to fill in depth for scenes. Our approach aligns the affine-invariant depth prior with metric-scale sparse measurements, enforcing them as hard constraints via an optimization loop at test-time. Our zero-shot depth completion method demonstrates generalization across various domain datasets, achieving up to a 21\% average performance improvement over the previous state-of-the-art methods while enhancing spatial understanding by sharpening scene details. We demonstrate that aligning a monocular affine-invariant depth prior with sparse metric measurements is a proven strategy to achieve domain-generalizable depth completion without relying on extensive training data. Project page: https://hyoseok1223.github.io/zero-shot-depth-completion/.

==> Figures/r-ssim.tex <==
\begin{figure}[!t]
\centering
   \includegraphics[width=1.0\linewidth]{Figures/r-ssim_arxiv.pdf}
   \caption{\textbf{Qualitative ablation of R-SSIM loss.}
    This structural regularization sharpens details in areas such as signposts and car shapes.
   } 
\label{fig:r-ssim}
\end{figure}

==> Tables/ablation_loss.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Ablation Study on R-SSIM Loss.}}
\label{tab:ablation_loss}
\renewcommand{\arraystretch}{1.1} % Adjust the row height factor
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{m{2.5cm} cc cc}
    \toprule
    \multirow{2}[2]{*}{Method} & \multicolumn{2}{c}{KITTI DC} & \multicolumn{2}{c}{VOID} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
    & RMSE & MAE & RMSE & MAE\\
    \midrule
    Ours w/o R-SSIM & 1.6105 & 0.4061 & 0.1255 & 0.0469\\
    Ours w/ R-SSIM & 1.5023 & 0.4099 & 0.1116 & 0.0447\\
    \bottomrule
    \end{tabular}
    }
\end{table}


==> Tables/ablation_method.tex <==
\begin{table}[t]
\centering

\renewcommand{\arraystretch}{1.3} % Adjust the row height factor
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{ccc  cc cc}
    \toprule
    \multirow{2}[2]{*}{\makecell{Sampling \\ Method}} &\multirow{2}[2]{*}{\makecell{R-SSIM \\ Loss}} & \multirow{2}[2]{*}{\makecell{Outlier \\ Filtering}} & \multicolumn{2}{c}{KITTI DC} & \multicolumn{2}{c}{VOID} \\
    \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
     & & & RMSE & MAE & RMSE & MAE\\
    \midrule
    Naïve & & & 3.514 & 1.942 & 0.199 & 0.130\\
    Guided & & & 2.113 & 0.801 & 0.210 & 0.138\\ 
    % Guided Sampling + LORA~\cite{bansal2024universal, hu2022lora} & \textbf{1.4819} & 0.4463 \\ 
    Ours & & & 1.610 & 0.406 & 0.125 & 0.046 \\
    Ours & {\cmark} & & 1.502 & 0.409 & 0.111 & 0.044 \\
    Ours & {\cmark} & {\cmark} & 1.413 & 0.397 & 0.112 & 0.045\\
    \bottomrule
    \end{tabular}
    }
% \setlength{\abovecaptionskip}{2pt}
   \vspace{-3pt}
\caption{\textbf{Ablation studies.} We ablate our proposed methods including test-time alignment, R-SSIM loss, and prior-based outlier filtering, to demonstrate their effectiveness. 
% in zero-shot depth completion.
}
\label{tab:ablation_method}
% \vspace{-15pt}
\end{table}


==> supp_figures/scenenet.tex <==
\begin{figure*}[t]
\centering
   \includegraphics[width=0.85\linewidth]{supp_figures/scenenet_arxiv.pdf}
   \caption{\textbf{Qualitative results on SceneNet}} 
\label{fig:qual_scenenet}
\end{figure*}

==> supp_figures/waymo.tex <==
\begin{figure*}[t]
\centering
   \includegraphics[width=0.9\linewidth]{supp_figures/waymo_arxiv.pdf}
   \caption{\textbf{Qualitative results on Waymo}} 
\label{fig:qual_waymo}
\end{figure*}
